A Theoretical Understanding of Gradient Bias in Meta-Reinforcement Learning

Gradient-based Meta-RL (GMRL) refers to methods that maintain two-level optimisation procedures wherein the outer-loop meta-learner guides the inner-loop gradient-based reinforcement learner to achieve fast adaptations. In this paper, we develop a unified framework that describes variations of GMRL algorithms and points out that existing stochastic meta-gradient estimators adopted by GMRL are actually \textbf{biased}. Such meta-gradient bias comes from two sources: 1) the compositional bias incurred by the two-level problem structure, which has an upper bound of $\mathcal{O}\big(K\alpha^{K}\hat{\sigma}_{\text{In}}|\tau|^{-0.5}\big)$ \emph{w.r.t.} inner-loop update step $K$, learning rate $\alpha$, estimate variance $\hat{\sigma}^{2}_{\text{In}}$ and sample size $|\tau|$, and 2) the multi-step Hessian estimation bias $\hat{\Delta}_{H}$ due to the use of autodiff, which has a polynomial impact $\mathcal{O}\big((K-1)(\hat{\Delta}_{H})^{K-1}\big)$ on the meta-gradient bias. We study tabular MDPs empirically and offer quantitative evidence that testifies our theoretical findings on existing stochastic meta-gradient estimators. Furthermore, we conduct experiments on Iterated Prisoner's Dilemma and Atari games to show how other methods such as off-policy learning and low-bias estimator can help fix the gradient bias for GMRL algorithms in general.

==> __algo.tex <==
\begin{algorithm}[tbh]
	\caption{Gradient-based Meta-RL- statements in \textcolor{blue}{blue} refers only to Compositional bias correction, statements in \textcolor{red}{red} only to Hessian bias correction.}  
	\small
	\label{alg:main}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} $T,K$, stepsizes $\alpha$, initializations $\phi_0$ and $\theta_0$.
		\FOR{$t=0,1,2,...,T$}
		\STATE{Set $\hat{\boldsymbol{\theta}}_t^0 = \hat{\boldsymbol{\theta}}_{t-1}^{K} \mbox{ if }\; t> 0$ and $\theta_0$ otherwise 
		}
		\FOR{$i=0,....,K-1$}
		\STATE{Draw a sample batch $\tau^{i}_{t,0}$} and $\tau^{i}_{t,1}$ and $\tau^{i}_{t,2}$
		\vspace{0.05cm}
		\STATE{Update 
		$\hat{\boldsymbol{\theta}}_{t}^{i+1}=\hat{\boldsymbol{\theta}}_{t}^{0} + \alpha \nabla_{\boldsymbol{\theta}} \hat{J}^{\text{In}}(\phi_{t},\theta_{t}^{i},\{\tau_{t,0}^{i},\textcolor{blue}{\boldsymbol{\tau}_{0:t-1,0}^{i}}\})$
		}
		\STATE{Compute Jacobian {$\nabla_{\phi} \nabla_{\boldsymbol{\theta}} \hat{J}^{\text{In}}(\phi_{t},\theta_{t}^{i},\tau_{t,1}^{i})$}}
		\IF{$i >= 1$}
		\STATE{Compute Hessian {$ \nabla^{2}_{\boldsymbol{\theta}} \hat{J}^{\text{In}}(\phi_{t},\theta_{t}^{i},\tau_{t,2}^{i})$ }  \par or {\textcolor{red}{$ \nabla^{2}_{\boldsymbol{\theta}}
		\hat{J}_{\text{LVC}}^{\text{In}}(\phi_{t},\theta_{t}^{i},\tau_{t,2}^{i})$ }}} 
		%\textcolor{red}{with LVC} 
		%via Eq. \eqref{LVC_fix}
		%via Eq. \eqref{vanilla_PG}
		\ENDIF
		\ENDFOR
                 \STATE{Draw sample batches $\tau_3$ }
                 \STATE{Compute gradient {$\nabla_{\phi} \hat{J}^{\text{Out}}(\phi_{t},\theta_{t}^{K},\tau_3)$}}
                 \STATE{Compute gradient 
                 {$ \nabla_{\boldsymbol{\theta}} \hat{J}^{\text {Out}}(\phi_{t},\theta_{t}^{K},\tau_3)$}}
                 \STATE{ Compute meta-gradient estimate $\nabla\hat{J}(\phi_t)$ via Eq. \eqref{GMRL_estimate_gradient}}
                 \STATE{Update $\phi_{t+1}=\phi_t + \alpha \nabla \hat{J}^{K}(\phi_t) $}
		\ENDFOR
	\end{algorithmic}
	\end{algorithm}	
	\setlength{\textfloatsep}{5pt}% Remove \textfloatsep

